Energy Definition and Minimization in Avalanche Models for Solar Flares

Self-organised critical avalanche models are a class of cellular automata that, despite their simplicity, can be applied to the modeling of solar (and stellar) flares and generate robust power-law distributions in event size measures. However, bridging the conceptual gap to both magnetohydrodynamics and real flare observations continues to prove challenging. In this paper, we focus on a specific, key aspect of this endeavour, namely the definition of magnetic energy and its consequences for the model's internal dynamics and energy release statistics. We show that the dual requirement of releasing energy and restoring local stability demands that the instability criterion and boundary conditions be set in a manner internally consistent with a given energy definition, otherwise unphysical behavior ensues, e.g., negative energy release. Working with three energy definitions previously used in the literature, we construct such internally consistent avalanche models and compare/contrast their energy release statistics. Using the same set of models, we also explore a recent proposal by Farhang et al. (2018, 2019), namely that avalanches/flares should maximize the amount of energy released by the lattice when instabilities are triggered. This tends to produce avalanches of shorter duration but higher peak energy release, but adding up to similar total energy release. For the three energy definition we tested, such avalanche models exhibit almost identical distributions of event size measures. Our results indicate that the key to reproduce solar-like power-law slopes in these size measures is lattice configurations in which most nodes remain relatively far from the instability threshold.

==> Labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}


1 Section~\ref{S-Introduction}
    figure 1~\ref{fig:diffEnergies}
2 Section~\ref{S-EnergiesInDeterministic} 
3 Section~\ref{S-DynamicalImplications} 
4 Section~\ref{S-EnergyOptimization} 
5 Section~\ref{S-Predictability} 
6 Section~\ref{S-Discussion}
7 Section~\ref{S-Conclusion}

